Efficient Video Object Segmentation via Modulated Cross-Attention Memory

Recently, transformer-based approaches have shown promising results for semi-supervised video object segmentation. However, these approaches typically struggle on long videos due to increased GPU memory demands, as they frequently expand the memory bank every few frames. We propose a transformer-based approach, named MAVOS, that introduces an optimized and dynamic long-term modulated cross-attention (MCA) memory to model temporal smoothness without requiring frequent memory expansion. The proposed MCA effectively encodes both local and global features at various levels of granularity while efficiently maintaining consistent speed regardless of the video length. Extensive experiments on multiple benchmarks, LVOS, Long-Time Video, and DAVIS 2017, demonstrate the effectiveness of our proposed contributions leading to real-time inference and markedly reduced memory demands without any degradation in segmentation accuracy on long videos. Compared to the best existing transformer-based approach, our MAVOS increases the speed by 7.6x, while significantly reducing the GPU memory by 87% with comparable segmentation performance on short and long video datasets. Notably on the LVOS dataset, our MAVOS achieves a J&F score of 63.3% while operating at 37 frames per second (FPS) on a single V100 GPU. Our code and models will be publicly available at: https://github.com/Amshaker/MAVOS.

==> tables/Davis.tex <==
\begin{table}[ht]
\setlength{\tabcolsep}{3.2mm}
\centering
\footnotesize
\caption{Quantitative comparison with state-of-the-art models on DAVIS 2017 validation set. FPS is measured using V100 GPU.}
% \setlength{\tabcolsep}{4.0pt}
\begin{tabular}{l|ccc|c}
	
    \toprule
     Method & $\mathcal{J\&F}\uparrow$ & $\mathcal{J}\uparrow$ & $\mathcal{F}\uparrow$ & FPS $\uparrow$ \\
    \midrule
    CFBI~\cite{yan2020cfbi} &  81.9  & 79.3  & 84.5 &  5.9  \\
    SST~\cite{duke2021sstvos} &   82.5  & 79.9  & 85.1 & - \\
    CFBI+~\cite{yang2021cfbip} &  82.9  & 80.1  & 85.7  & 7.2 \\
    STCN~\cite{cheng2021stcn} &  85.4  & 82.2  & 88.6  & 19.5  \\
    RPCM~\cite{xu2022rpcm} &  83.7  & 81.3  & 86.0  & - \\
    
    DDMemory~\cite{voigtlaender2019feelvos} &  84.2 & 81.3 & 87.1 & 28.1\\
    XMem~\cite{cheng2022xmem} &  86.2 & 82.9 & 89.5 & 24.2\\
    AOT-L~\cite{yang2021aot}  & {83.8} & {81.1} & {86.4}  & 20.3 \\
    DeAOT-L~\cite{yang2022deaot} & {84.3} & {81.4} & {87.2}   &  {29.3}  \\
    
    \midrule
    % \rowcolor{LightCyan}
    \textbf{MAVOS (Ours)} & {84.4} & {81.5} & {87.2}  & {38.1}  \\
    % \rowcolor{LightCyan}
    \textbf{R50-MAVOS (Ours)} & {85.6} & {82.6} & {88.5}  & {35.0}  \\
    % \rowcolor{LightCyan}
    \textbf{SwinB-MAVOS (Ours)} & {86.4} & {83.2} & {89.6} & {21.8}   \\
    \bottomrule

\end{tabular}

\label{tab:davis}
\end{table}
